FastDrain: Removing Page Victimization Overheads in NVMe Storage Stack

Host-side page victimizations can easily overflow the SSD internal buffer, which interferes I/O services of diverse user applications thereby degrading user-level experiences. To address this, we propose FastDrain, a co-design of OS kernel and flash firmware to avoid the buffer overflow, caused by page victimizations. Specifically, FastDrain can detect a triggering point where a near-future page victimization introduces an overflow of the SSD internal buffer. Our new flash firmware then speculatively scrubs the buffer space to accommodate the requests caused by the page victimization. In parallel, our new OS kernel design controls the traffic of page victimizations by considering the target device buffer status, which can further reduce the risk of buffer overflow. To secure more buffer spaces, we also design a latency-aware FTL, which dumps the dirty data only to the fast flash pages. Our evaluation results reveal that FastDrain reduces the 99th response time of user applications by 84%, compared to a conventional system.

==> highlevelview.tex <==
%In this section, we first explain the high-level view of SimpleSSD that integrates our NVMe stack interface model, SSD firmware simulation and flash/device hardware abstraction framework, referred to as SimpleSSD. We then describe details of each simulation component/layer and discuss simulator's implementation issues.  


The proposed SimpleSSD executes a variety of OS binaries with Linux emulation, which can run all runtime libraries, real user applications, and the full storage stack. Thus, I/O requests that a user application generates can go through the full storage stack and visit all necessary kernel components, including the file system, page cache, blk-mq, and NVMe drivers. The requests are then served by realizing all necessary hardware and firmware components of a modern multi-channel/multi-way SSD architecture. 


\begin{figure}
	\centering	
	\includegraphics[width=1\linewidth]{figs/high_gem5HW}
	\vspace{-25pt}
	\caption{Overview of our simulation infrastructure. \vspace{-15pt}}
	\label{fig:high_gem5HW}
\end{figure}


\subsection{Overview}
\noindent \textbf{Holistic architecture.}
Figure \ref{fig:high_gem5HW} illustrates an overview of our simulation architecture from a holistic viewpoint. CPU cores (e.g., x86/ARM), including multiple on-chip cache memories, are simulated by gem5. This computation part simulates architectural components and emulates Linux system, which is connected to SimpleSSD over the PCI/PCIe system bus. Specifically, as shown in the figure, a specific memory address range, called the on-chip peripherals memory region, is mapped to a set of registers that SimpleSSD's controller/firmware exposes. This memory region includes two memory spaces, the PCIe configuration space and the PCIe memory space. The PCIe configuration space enables the underlying SimpleSSD (per device) to provide PCIe device descriptions, such as a vendor identification (ID) number and device ID, version ID, and so forth, whereas the PCIe memory space maps registers related to the SSD's I/O service. SimpleSSD simulates multiple flash packages that consist of multiple dies and planes, based on user's configuration, and such packages are connected to multiple DRAM modules and controllers. 


\noindent \textbf{SSD firmware simulation.} A challenge in simulating an SSD is to support different flash firmware versions, which greatly influences the target storage performance. We model a flexible \emph{flash translation layer} (FTL) whose address translation mechanism can be easily reconfigured based on different associativity granularities that the system architects define. We also decouple the I/O scheduling and page allocation mechanisms from FTL, such that new scheduling proposals, that are aware of SSD-internal parallelism, can be embedded without changing the FTL. Note that, although we do not cover all potential variations that can be observed in industrial FTLs, the implemented reconfigurable mapping algorithm can capture and support diverse operational characteristics of a block/page-level mapping FTL, fully-associative FTL, and various hybrid mapping schemes that employ different levels of block and page mapping tables in address translations. 

\noindent \textbf{Device hardware abstraction.} The performance characteristics of an SSD device vary according to i) the latency intrinsics of individual flash characteristics and ii) their different levels of parallelism. 
In this work, we abstract both flash-level and subsystem-level hardware characteristics, and we implemented an FPGA-based memory controller built upon Xilinx Spartan-6 \cite{alfke2009xilinx} and characterized different memory technologies. Based on the extracted characteristics, we first design a die-level latency model and incorporate it into flash transaction scheduling. Specifically, we examine all the flash transactions specified by the open NAND flash interface (ONFi 3.x \cite{workgroup2011open}), and classify various timing components of the corresponding protocol into schedulable transaction activities. This low-level abstraction can capture close interactions across the firmware, controller and architecture designs by being aware of flash latency intrinsics and internal parallelism.  


\begin{figure}
	\centering	
	\includegraphics[width=1\linewidth]{figs/high_nvmeq}
	\vspace{-25pt}
	\caption{NVMe queue management.\vspace{-15pt}}
	
	\label{fig:high_nvmeq}
\end{figure}


\subsection{NVMe Stack}
\noindent \textbf{NVMe command and queue.} 
Figure \ref{fig:high_nvmeq} illustrates the NVMe queue element (command) and management mechanism. Specifically, the I/O requests coming from mq-blk in the low-level of SimpleSSD are managed by NVMe submission queue (SQ) and completion queue (CQ) elements. Each queue element is encoded to a 64 byte PCIe packet, and can contain a command ID, an operation code (\emph{opcode}) and physical region pages (\emph{PRPs}). When the NVMe driver receives an NVMe command from upper side of software in storage stack over \texttt{nvme\_rw\_command}, the driver embeds the type of requests such as a read or a write, into its opcode, and composes PRPs by filling the system kernel addresses that refer actual data contents associated with the corresponding I/O request to each entry (per 4KB). This NVMe command is issued to the target SQ, which can accommodate 65,536 queue entries. A new NVMe command is always appended at the end of a queue, which is referred by a tail pointer, while a head pointer points to the oldest entry of the queue. Thus, once the command is successfully enqueued, the NVMe driver increases the SQ's tail pointer and informs it to the underlying NVMe controller of SimpleSSD by writing the tail doorbell register. Once SimpleSSD completes the request simulation (per NVMe entry), it enqueues a complete NVMe command (which has a completion tag) into the CQ paired by the target SQ by writing its system memory, and it interrupts the NVMe driver through a message-signalled interrupt (MSI).  Note that, since NVMe specifications define per-core many NVMe queues (65,536 queues), each being paired by an SQ and a CQ, the I/O completion is enqueued into the corresponding CQ by SimpleSSD side NVMe controller. 
The driver then checks the tag field of all CQ's commands located between the head and tail pointers, and it increases the tail pointer whenever the driver finds a completion tag. After that, the NVMe driver calls the corresponding I/O completion routine of the storage stack, so that users can receive an appropriate service. Finally, as an NVMe tear-down process, the driver cleans up the queue entry (for SQ/CQ) and increments the head pointer and informs it again to the underlying NVMe controller of SimpleSSD. 


\begin{figure}
	\centering	
	\includegraphics[width=1\linewidth]{figs/high_interact}
	\vspace{-25pt}
	\caption{NVMe interface and controller. \vspace{-15pt}}
	\label{fig:high_interact}
\end{figure}

\begin{figure*}
%\vspace{-10pt}
\centering{}\includegraphics[width=1\columnwidth]{figs/simplessd-arch}
\vspace{-25pt}
\caption{High-level veiw of SimpleSSD.\label{fig:HIL}\vspace{-15pt}} 
\end{figure*}

\noindent \textbf{NVMe interface and controller.}
Figure \ref{fig:high_interact} shows the details of the NVMe interface that SimpleSSD uses to connect the NVMe driver (gem5 side) and the NVMe controller (SimpleSSD side). Based on the address of BAR that the number driver writes, SimpleSSD hooks the event and simulates such PCIe communication by calling the NVMe controller's \texttt{ringSQTailDoorbell()} and \texttt{ringCQHeadDoorbell()}.  While \texttt{ringSQTailDoorbell()} is related to increasing the SQ's tail pointer by writing the tail doorbell register, \texttt{ringCQHeadDoorbell()} increases the value of the CQ's head pointer by emulating the function of writing the head doorbell register. Since each NVMe queue entry (i.e., command) contains an opcode and PRPs, the NVMe controller can know the locations of the system memory regions that SimpleSSD needs to bring in the target data. The NVMe controller performs actual data transfers (for the request) by looking up the PRP list that the NVMe driver in the storage stack generated from the gem5 side. When the controller informs the NVMe driver of an I/O completion, the process of posting an MSI or MSI extension (MSI-X) is simulated by \texttt{updateInterrupt()} of our controller. In addition, the controller also simulates the functions related to NVMe register reads and writes through \texttt{readRegister()} and \texttt{writeRegister()}, respectively. Using these functions, the NVMe driver can understand the status of the NVMe controller and firmware if it needs to. With this NVMe interface and queue simulation method, our NVMe controller can convert all NVMe entries to I/O requests and flash transactions, which are used within our SSD simulation model. Generally speaking, a request is first taken by the host interface layer (HIL), and the corresponding target address is translated by FTL. After that, the parallelism allocation layer (PAL) services the request by abstracting the physical layout of interconnection buses and flash dies. The completion of an I/O request is reported from PAL to HIL, and is posted to the NVMe driver through the NVMe controller. 

Note that our simulation infrastructure actually shows physical NVMe device(s) and storage volume(s) for users under OS's \texttt{/dev/}. Each I/O request reflects all system behaviors, various controller/firmware specific execution times, and flash-level memory latency in SimpleSSD, which can capture very detailed information of NVMe-based SSD subsystems as well. This SimpleSSD simulation methodology is completely different from those employed by existing SSD simulators, which require block-level I/O traces to be replayed for their workload execution. 


\subsection{Fully-Functional Firmware Simulation}

\noindent \textbf{Host interface layer.} 
Figure \ref{fig:HIL} presents the internal process of SimpleSSD. In SimpleSSD, HIL first receives an incoming request from the NVMe controller and enqueues the request in a device-level queue. During this phase, it parses the host-side information and translates it a LBA, request type, number of sectors, and a host's system time information (e.g., tick). HIL then forwards this translated information to the underlying FTL through communication APIs, \texttt{ReadTransaction()} and \texttt{WriteTransaction()}. During this phase, HIL also accesses the internal DRAM for buffering/transferring the data and scheduling I/O requests, being aware of the status of underlying firmware modules or hardware components. 

%Since there are many different types of simulation models for a full system (e.g., discrete event-driven, activity-driven and continuous), HIL exposes all request completions through a latency map table, which includes the finish time (i.e., finishTick) along with each requested address. 
%One of the things that HIL needs to take into account is the different simulation domains between a full system simulator and our SSD simulation model. For example, while the execution of an instruction can be stalled in cases where it accesses the underlying SSD (because of a cache miss or system call), the actual full system simulation should not be halted due to I/O service model. 
%To address this issue, HIL employs a latency map table that includes the completion time for each requested address. 
%Once the latency for each request is updated by the underlying simulation modules, HIL updates the table with the completion time, and the full-system simulator (e.g., gem5) retrieves it in an asynchronous fashion. While the current queue implementation of HIL is first-come-first-served, system and computer architects can insert their buffer cache, I/O reordering logic, or scheduler into HIL.



\noindent \textbf{Flash translation layer.}
%While a host can send an I/O request whose size varies based on the decision of a full system simulator's file system or traces 
%all actual services at flash level should be performed by page granularity. 
The I/O sizes requested by a host application vary and can be even larger than the page size that a single flash die could accommodate.  
Therefore, in this work, FTL separates each request forwarded by HIL into multiple \emph{sub-requests}, each indicated by a logical page number (LPN). If it is a read, FTL directly translates the sub-requests' LPNs to PPNs by looking up its own address mapping table. 
Otherwise, FTL allocates new page(s) and updates the table with appropriate block and/or page addresses and other meta-data information. 
In SimpleSSD, this address translation mechanism is implemented in a functional API, called \texttt{FTLmapping()}. 
The translated or allocated PPNs are then issued into the underlying module's queue by calling \texttt{SendRequest()}, and FTL repeats this process until there is no waiting sub-request. 
When there is no available page for a write, FTL performs a GC to reclaim a set of new pages in flash block(s). 
At the beginning of GC, it selects the victim blocks and free block(s) to allocate as a new block, which can be determined by a wear-leveling algorithm. After this selection, FTL reads the data from all valid pages of the victim blocks, writes them into the new block,  and updates the address table for the reclaimed blocks. Note that the additional read and write operations imposed by GC(s) are treated just like other sub-requests as far as FTL is concerned in SimpleSSD. 
In this work, we consider a simple GC algorithm called the greedy algorithm \cite{bux2010performance}, which selects the block with the maximum number of invalid pages as a \textit{victim}. 
Besides, the wear-leveling algorithm that we implement always allocates new block(s) by considering the minimum erase count among the free blocks in a reserved pool. Users can replace these algorithms by updating  \texttt{GarbageCollection()} and \texttt{WearLeveling()}. 



\subsection{Hardware Simulation for Scalable SSD Parallelism}

\noindent \textbf{Parallelism abstraction layer.}
From a functionality perspective, the key role of FTL is to translate addresses, while not managing different levels of parallelism (explained earlier in Section \ref{sec:ssd}) or flash transactions. We introduce PAL underneath FTL, which decouples SSD parallelism from other flash firmware modules for simulation efficiency. At the beginning, PAL dequeues the requests issued by FTL and disassembles the target page address by being aware of the underlying hardware configuration (e.g., the numbers of channels, flash packages and dies), which is implemented in \texttt{PPNdisassemble()}.
Based on the disassembled information, PAL simulates SSD internal state and schedules the flash transactions at a finer granularity, which can capture memory-specific latency, idle time and even scheduling penalties imposed by resource contentions. In other words, the latency of a sub-request can be dynamically simulated by considering not only the hardware resource availability but also the storage media configuration in SimpleSSD. Completing the processing of an I/O request, PAL returns the simulated latency for each sub-request to FTL. FTL then collects and re-evaluates them to generate the appropriate latency of the I/O request that possess such sub-requests. By being aware of the states of the underlying hardware, users can explore new parallelism strategies and schedulers, which determine the order of sub-request stripping or manage flash transactions with a modification of \texttt{PPNdisassemble()} and  \texttt{TimelineScheduling()} implemented in this layer, respectively.



%\begin{table}
%\centering
%\resizebox{\textwidth}{!}{
%\caption{Configurations for system simulations.}
%\label{tab:sys_config}
%\begin{tabular}{|c|c|c|c|c|c|l|}
%\hline
%\textbf{Channel} & \textbf{Package} & \textbf{Die} & \textbf{Plane} & \textbf{Block} & \textbf{CPU} & ARMv7, 1 core, 1GHz \\ \hline
%8 & 8 & 4 & 2 & 1024 & \multirow{2}{*}{\textbf{Cache}} & L1I\$/L1D\$, 64KB, 4-way \\ \cline{1-5} \cline{7-7} 
%\textbf{DMA(MHz)} & \textbf{Pages/blk} & \textbf{Page} & \textbf{OP} & \textbf{GC} &  & L2\$, 512KB, 8-way \\ \hline
%400 & 256 & 8KB & 0.2 & 0.05 & \textbf{DRAM} & DDR3, 1 channel, 2 rank \\ \hline
%\end{tabular}}
%\vspace{-10pt}
%\end{table}


%\subsection{Enabling Full System Simulation}

\noindent \textbf{Latency variation mapping.}
To increase storage density while staying within the same transistor budget, flash can store multiple states in a single storage cell. 
For example, \emph{triple-level cell} (TLC) flash stores eight different states into a target storage core, and each of the states is represented by different voltage thresholds ($V_{th}$). Since a TLC core can maintain 3-bit data, the TLC technology can drastically increase the storage capacity of an SSD. However, the materials of the TLC storage core are not fundamentally different from those of a \emph{single-level cell} (SLC) or \emph{multiple-level cell} (MLC), which can represent 1-bit or 2-bit data per cell, respectively. Instead, the flash logic of TLC (and MLC) writes (also known as programs) data into a target in a different manner than SLC flash. This is referred to as an \emph{increment step pulse program} (ISPP \cite{suh19953}), which introduces significant latency variation.
To characterize the latency behavior incurred by an ISPP, we built an FPGA-based controller using Xilinx Spartan-6 and tested SLC, MLC, and TLC NAND flash devices.  Figures \ref{figs:readlatency} and \ref{figs:writelatency} illustrate the latency variation observed for writes and reads, respectively, on TLC 25 nm flash technology \cite{TLC-NAND}. We provide only the results for TLC due to the page limit, but other flash technologies exhibit the same latency trend on that we observed for TLC. The evaluation data are measured in every single block and page. For writes, the latency of the \emph{most significant bit} (MSB) pages is longer than that of the \emph{center significant bit} (CSB) and \emph{least significant bit} (LSB) pages by approximately 1.3 and 8 times, respectively. 
%The reason why there exists the significant latency disparity among LSB/CSB/MSB is that TLC flash preforms many verify-and-program steps (of ISPP) to generate an accurate voltage distribution on the target. However, each state of TLC flash has a very tight $V_{th}$ margin as considering that it puts eight states into a single cell, and therefore, such verify-and-program process introduce a number of reads and programs to write appropriate data. 
The reads on TLC flash also exhibit similar latency variation characteristics. Specifically, the read latency of MSB pages is longer than that of CSB pages and LSB pages by 37\% and 84\%, on average, respectively. 
%This is because flash control logic (within a chip) requires to check the target state by shifting and applying the reference voltages till to find out the target. Thus, the number of checks on MSB pages is greater than that of CSB pages and LSB pages. 
Since the latencies between different pages exhibit a notable difference, this can have a great impact on parallelism and hardware modelling. We observe that the first five pages within a block always exhibit LSB page performance, and the latency of next three pages (after the first five) is the same as that of the CSB pages. 
These eight pages, referred to as \emph{meta pages}, are usually used for storing the metadata of flash firmware such as mapping information associated with the block. 
The latency for all the remaining pages can be mapped by following the simple function: $f(addr) = (addr - n_{meta}) / n_{plane} \bmod n_{state}$ where $addr$, $n_{meta}$, $n_{state}$ and $n_{plane}$ are the input address, the number of meta pages, the number of states per cell, and the number of planes within a flash die, respectively. If $f(addr)$ is 0, it is an LSB page, and if $f(addr)$ is 1, it is a CSB page. Otherwise, the address indicates an MSB page.

Note that, as shown in Figure \ref{figs:writelatency}, while most blocks follow the aforementioned latency function, we observe that a few blocks (e.g., blocks 7 and 15) exhibit an abnormal latency distribution. This is because, a few blocks can be defective in the process of manufacturing or get damaged with heavy program tests, called \emph{bad blocks}. As a flash controller cannot correctly program the cells of such bad blocks, the program latency for their individual pages can be different from the latency for pages of other normal blocks.

\begin{figure}
\centering
%\subfloat[ISPP.]{\label{figs:readlatency}\rotatebox{0}{\includegraphics[width=0.24\linewidth]{figs/ispp-vth}}}
%\hspace{1pt}
%\subfloat[TLC Programming.]{\label{figs:readlatency}\rotatebox{0}{\includegraphics[width=0.24\linewidth]{figs/ispp-dist}}}
%\hspace{1pt}
\subfloat[Read latency.]{\label{figs:readlatency}\rotatebox{0}{\includegraphics[width=0.49\linewidth]{figs/readlatency}}}
\hspace{1pt}
\subfloat[Write latency.]{\label{figs:writelatency}\rotatebox{0}{\includegraphics[width=0.49\linewidth]{figs/writelatency}}}
\vspace{-7pt}
\caption{\label{fig:latency}Analysis for flash intrinsic latency variation.\vspace{-7pt}}
\end{figure}


%\section{Model Implementation}
%\label{sec:implementation}
%\input{implementation}

